JavaBench: A Benchmark of Object-Oriented Code Generation for Evaluating Large Language Models

Code generation benchmarks such as HumanEval are widely adopted to evaluate LLMs' capabilities. However, after consolidating the latest 24 benchmarks, we noticed three significant imbalances. First, imbalanced programming language. 95.8% of benchmarks involve Python, while only 5 benchmarks involve Java. Second, imbalanced code granularity. Function-/statement-level benchmarks account for over 83.3% of benchmarks. Only a mere handful extends to class-/project-levels, and all are limited to Python. Third, lacking advanced features. Existing benchmarks primarily assess basic coding skills, while overlooking advanced Object-Oriented Programming (OOP) features (i.e., encapsulation, inheritance, and polymorphism). To fill these gaps, we propose JavaBench, a project-level Java benchmark that exercises OOP features. It comprises four Java projects with 389 methods in 106 Java classes. The test coverage is up to 92%, and JavaBench is attested by 282 undergraduate students, reaching a 90.93/100 average score (i.e., pass rate against the test suite), ensuring the quality of documentation, code skeleton, and tests. To better evaluate LLM's capability against JavaBench, we introduce a systematic evaluation design covering three context settings and five synthesis strategies at two granularities using three hierarchical metrics. Our extensive experiment yields several interesting findings. First, we noticed that regarding project-level Java programming, LLMs are far behind undergraduate students (no project can be correctly completed by any studied LLMs, and at most 41.17% Pass@5 in a more relaxed evaluation). Second, using method signature as prompt context may strike an ideal balance for project-level code generation. JavaBench is publicly available at https://github.com/java-bench/JavaBench.

==> Code/fail-exception.tex <==
public class ConsolePlayer {
  public Move nextMove(Game game, Move[] availableMoves) {
    ...
|\textbf{\textcolor{teal}{+}}|   try {
      Scanner in = new Scanner(System.in);
      String source = in.nextLine().toLowerCase();
      int sourceX = source.chatAt(0) - 'a';
      // There is uncertainty in user input. 
      // And failure to handle NumberFormatException will cause the program to crash directly.
      int sourceY = Integer.parseInt(source.substring(1)) - 1; 
      ...
|\textbf{\textcolor{teal}{+}}|   } catch(...) { ... }
  }
}

==> Code/fail-initial.tex <==
public class FillableCell extends Cell {
  private Pipe pipe;
  
  public FillableCell(Coordinate coord) {
    super(coord);
    pipe = null;
  }
  
  public FillableCell(Coordinate coord, Pipe pipe) {
    super(coord);
    // Should be initiated: this.pipe = pipe
    pipe = null;
    this.pipe = pipe;
  }
}

==> FigureTex/prompt.tex <==
\begin{figure}[t]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=0.7\linewidth]{./Figure/prompt.pdf}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Prompt Template used in the Experiment}
    \label{fig:prompt}
\end{figure}

==> FigureTex/workflow.tex <==
\begin{figure*}[t]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=1.0\linewidth]{./Figure/workflow.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Workflow (Draft)}
    \label{fig:workflow}
\end{figure*}

==> Listing/listing-fail-exception.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}

\begin{figure}[h!]
	\lstinputlisting[
		language=java,
        % basicstyle=\linespread{0.8}\tiny,
        % baselinestretch=1.0,
		% morekeywords={var},
            % aboveskip=-2pt,
            % belowskip=-2pt,
		% caption={\textbf{Prompt Template used in the Experiment}},
		% label={listing:prompt},
		escapechar=|,
  		linebackgroundcolor = {
                \ifnum \value{lstnumber} = 4 \color{added} \fi
                \ifnum \value{lstnumber} = 12 \color{added} \fi
            },
		numbers=left
	]{./Code/fail-exception.tex}
\end{figure}



==> Listing/listing-fail-init.tex <==

\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
	\lstinputlisting[
		language=java,
        % basicstyle=\linespread{0.8}\tiny,
        % baselinestretch=1.0,
		% morekeywords={var},
            % aboveskip=-2pt,
            % belowskip=-2pt,
		% caption={\textbf{Prompt Template used in the Experiment}},
		% label={listing:prompt},
		escapechar=|,
		% linebackgroundcolor = {\ifnum \value{lstnumber} > 2 \ifnum \value{lstnumber} < 10 \color{stubbg} \fi \fi},
		numbers=left
	]{./Code/fail-initial.tex}
\end{figure}



==> Table/completion.tex <==

\begin{table}[t!]
\centering
\caption{Results of Completion@K.}
\label{tab:compilation}
\renewcommand\arraystretch{1.2}
    \resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|l|llll}
\toprule
Synthesis & Model & P1 & P2 & P3 & P4 \\
\midrule
Holistic & WizardCoder-15B & \cellcolor[HTML]{97C5B2}90.00\% & \cellcolor[HTML]{C1DDD1}62.86\% & \cellcolor[HTML]{90C1AD}94.29\% & \cellcolor[HTML]{B4D5C7}71.43\% \\
Holistic & deepseek-6.7b & \cellcolor[HTML]{9AC7B4}88.00\% & \cellcolor[HTML]{9CC8B5}87.14\% & \cellcolor[HTML]{87BCA6}100.00\% & \cellcolor[HTML]{87BCA6}100.00\% \\
Holistic & deepseek-33b & \cellcolor[HTML]{87BCA6}100.00\% & \cellcolor[HTML]{AFD3C4}74.29\% & \cellcolor[HTML]{87BCA6}100.00\% & \cellcolor[HTML]{87BCA6}100.00\% \\
Holistic & Phind-34B & \cellcolor[HTML]{9AC7B4}88.00\% & \cellcolor[HTML]{A7CEBE}80.00\% & \cellcolor[HTML]{97C5B2}90.00\% & \cellcolor[HTML]{A7CEBE}80.00\% \\
Holistic & gpt-3.5-turbo-1106 & \cellcolor[HTML]{97C5B2}90.00\% & \cellcolor[HTML]{A0CAB9}84.29\% & \cellcolor[HTML]{87BCA6}100.00\% & \cellcolor[HTML]{90C1AD}94.29\% \\
\hline
Independent & WizardCoder-15B & \cellcolor[HTML]{ADD1C2}76.00\% & \cellcolor[HTML]{BBD9CC}67.14\% & \cellcolor[HTML]{B6D7C9}70.00\% & \cellcolor[HTML]{FBFDFC}25.71\% \\
Independent & deepseek-6.7b & \cellcolor[HTML]{BCDACE}66.00\% & \cellcolor[HTML]{97C5B2}90.00\% & \cellcolor[HTML]{8CBFAA}97.14\% & \cellcolor[HTML]{9EC9B7}85.71\% \\
Independent & deepseek-33b & \cellcolor[HTML]{B3D5C7}72.00\% & \cellcolor[HTML]{C1DDD1}62.86\% & \cellcolor[HTML]{93C3AF}92.86\% & \cellcolor[HTML]{87BCA6}100.00\% \\
Independent & Phind-34B & \cellcolor[HTML]{E8F2EE}38.00\% & \cellcolor[HTML]{ABD0C1}77.14\% & \cellcolor[HTML]{B8D8CB}68.57\% & \cellcolor[HTML]{B4D5C7}71.43\% \\
Independent & gpt-3.5-turbo-1106 & \cellcolor[HTML]{97C5B2}90.00\% & \cellcolor[HTML]{99C6B4}88.57\% & \cellcolor[HTML]{95C4B0}91.43\% & \cellcolor[HTML]{B4D5C7}71.43\% \\
\hline
Incremental & WizardCoder-15B & \cellcolor[HTML]{B9D8CB}68.00\% & \cellcolor[HTML]{BFDCD0}64.29\% & \cellcolor[HTML]{DAEAE3}47.14\% & \cellcolor[HTML]{FFFFFF}22.86\% \\
Incremental & deepseek-6.7b & \cellcolor[HTML]{B6D7C9}70.00\% & \cellcolor[HTML]{9EC9B7}85.71\% & \cellcolor[HTML]{8ABEA8}98.57\% & \cellcolor[HTML]{95C4B0}91.43\% \\
Incremental & deepseek-33b & \cellcolor[HTML]{C9E1D7}58.00\% & \cellcolor[HTML]{BFDCD0}64.29\% & \cellcolor[HTML]{95C4B0}91.43\% & \cellcolor[HTML]{9EC9B7}85.71\% \\
Incremental & Phind-34B & \cellcolor[HTML]{DFEDE7}44.00\% & \cellcolor[HTML]{ADD2C3}75.71\% & \cellcolor[HTML]{BDDACE}65.71\% & \cellcolor[HTML]{CFE4DB}54.29\% \\
Incremental & gpt-3.5-turbo-1106 & \cellcolor[HTML]{B6D7C9}70.00\% & \cellcolor[HTML]{9EC9B7}85.71\% & \cellcolor[HTML]{99C6B4}88.57\% & \cellcolor[HTML]{95C4B0}91.43\% \\
\bottomrule
\end{tabular}
}
\end{table}

==> Table/rq3.tex <==

\begin{table*}[t!]
\centering
\caption{RQ2 -- Performance Variance Over Different Context Settings.}
\label{tab:rq3}
\renewcommand\arraystretch{1.2}
    \resizebox{1.0\textwidth}{!}{
\begin{tabular}{ll|llll||llll||llll||llll||llll}
\toprule
 &  & \multicolumn{4}{c}{} & \multicolumn{8}{c}{\textbf{Compilation @ 1}} & \multicolumn{8}{c}{\textbf{Pass @ 1}} \\
 &  & \multicolumn{4}{c}{\multirow{-2}{*}{\textbf{Completion @ 1}}} & \multicolumn{4}{c}{\textbf{class-wise}} & \multicolumn{4}{c}{\textbf{test-wise}} & \multicolumn{4}{c}{\textbf{class-wise}} & \multicolumn{4}{c}{\textbf{test-wise}} \\ 
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c|}{\textbf{Incremental Strategy}} & \multicolumn{1}{c}{\textbf{P1}} & \multicolumn{1}{c}{\textbf{P2}} & \multicolumn{1}{c}{\textbf{P3}} & \multicolumn{1}{c}{\textbf{P4}} & \multicolumn{1}{c}{\textbf{P1}} & \multicolumn{1}{c}{\textbf{P2}} & \multicolumn{1}{c}{\textbf{P3}} & \multicolumn{1}{c}{\textbf{P4}} & \multicolumn{1}{c}{\textbf{P1}} & \multicolumn{1}{c}{\textbf{P2}} & \multicolumn{1}{c}{\textbf{P3}} & \multicolumn{1}{c}{\textbf{P4}} & \multicolumn{1}{c}{\textbf{P1}} & \multicolumn{1}{c}{\textbf{P2}} & \multicolumn{1}{c}{\textbf{P3}} & \multicolumn{1}{c}{\textbf{P4}} & \multicolumn{1}{c}{\textbf{P1}} & \multicolumn{1}{c}{\textbf{P2}} & \multicolumn{1}{c}{\textbf{P3}} & \multicolumn{1}{c}{\textbf{P4}} \\

\midrule
deepseek-coder-6.7b-instruct & Forward & \cellcolor[HTML]{ABD0C0}70.00\% & \cellcolor[HTML]{98C5B2}85.71\% & \cellcolor[HTML]{88BCA7}98.57\% & \cellcolor[HTML]{91C1AD}91.43\% & \cellcolor[HTML]{ABD0C0}70.00\% & \cellcolor[HTML]{ACD1C1}68.57\% & \cellcolor[HTML]{9BC7B5}82.86\% & \cellcolor[HTML]{ACD1C1}68.57\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{AACFC0}70.59\% & \cellcolor[HTML]{D5E8E0}34.29\% & \cellcolor[HTML]{ADD1C2}67.59\% & \cellcolor[HTML]{AED1C2}67.43\% & \cellcolor[HTML]{9CC7B5}82.15\% & \cellcolor[HTML]{B1D3C5}64.30\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{AACFC0}70.59\% & \cellcolor[HTML]{F5F9F7}8.12\% \\
deepseek-coder-6.7b-instruct & Reverse & \cellcolor[HTML]{AFD2C4}66.00\% & \cellcolor[HTML]{93C2AE}90.00\% & \cellcolor[HTML]{8ABDA8}97.14\% & \cellcolor[HTML]{A2CBBA}77.14\% & \cellcolor[HTML]{AFD2C4}66.00\% & \cellcolor[HTML]{A9CFBF}71.43\% & \cellcolor[HTML]{9FC9B7}80.00\% & \cellcolor[HTML]{BAD8CC}57.14\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{F6FAF8}7.27\% & \cellcolor[HTML]{AACFC0}70.59\% & \cellcolor[HTML]{E0EDE8}25.71\% & \cellcolor[HTML]{B2D4C6}63.59\% & \cellcolor[HTML]{ACD0C1}69.07\% & \cellcolor[HTML]{9FC9B8}79.60\% & \cellcolor[HTML]{BEDACF}53.77\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{F9FBFA}4.92\% & \cellcolor[HTML]{AACFC0}70.59\% & \cellcolor[HTML]{F5F9F7}7.91\% \\
deepseek-coder-6.7b-instruct & Random & \cellcolor[HTML]{A8CEBE}72.00\% & \cellcolor[HTML]{93C2AE}90.00\% & \cellcolor[HTML]{8CBEA9}95.71\% & \cellcolor[HTML]{9BC7B5}82.86\% & \cellcolor[HTML]{ADD1C2}68.00\% & \cellcolor[HTML]{ABD0C0}70.00\% & \cellcolor[HTML]{9FC9B7}80.00\% & \cellcolor[HTML]{B7D6C9}60.00\% & \cellcolor[HTML]{EDF4F1}15.00\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{B4D5C7}62.35\% & \cellcolor[HTML]{E3EFEA}22.86\% & \cellcolor[HTML]{B0D3C4}65.56\% & \cellcolor[HTML]{ACD1C2}68.43\% & \cellcolor[HTML]{9FC9B8}79.63\% & \cellcolor[HTML]{B8D7CA}59.04\% & \cellcolor[HTML]{EDF5F2}14.40\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{B4D5C7}62.06\% & \cellcolor[HTML]{F5F9F8}7.85\% \\
\hline
gpt-3.5-turbo-1106 & Forward & \cellcolor[HTML]{ABD0C0}70.00\% & \cellcolor[HTML]{98C5B2}85.71\% & \cellcolor[HTML]{94C3B0}88.57\% & \cellcolor[HTML]{91C1AD}91.43\% & \cellcolor[HTML]{B7D6C9}60.00\% & \cellcolor[HTML]{9FC9B7}80.00\% & \cellcolor[HTML]{A9CFBF}71.43\% & \cellcolor[HTML]{ACD1C1}68.57\% & \cellcolor[HTML]{F0F6F3}12.50\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{E0EDE8}25.71\% & \cellcolor[HTML]{B9D8CB}57.80\% & \cellcolor[HTML]{9FC9B7}79.80\% & \cellcolor[HTML]{A9CFBF}71.43\% & \cellcolor[HTML]{B1D3C5}64.84\% & \cellcolor[HTML]{F0F6F3}12.50\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{F5F9F7}8.10\% \\
gpt-3.5-turbo-1106 & Reverse & \cellcolor[HTML]{9AC6B4}84.00\% & \cellcolor[HTML]{94C3B0}88.57\% & \cellcolor[HTML]{A1CAB9}78.00\% & \cellcolor[HTML]{A5CDBC}74.29\% & \cellcolor[HTML]{9FC9B7}80.00\% & \cellcolor[HTML]{9DC8B6}81.43\% & \cellcolor[HTML]{C3DDD2}50.00\% & \cellcolor[HTML]{BDDACE}54.29\% & \cellcolor[HTML]{BAD8CB}57.50\% & \cellcolor[HTML]{E9F2EE}18.18\% & \cellcolor[HTML]{E5F0EC}21.18\% & \cellcolor[HTML]{FFFFFF}0.00\% & \cellcolor[HTML]{A0CAB9}78.46\% & \cellcolor[HTML]{A0CAB8}78.88\% & \cellcolor[HTML]{C3DDD2}50.00\% & \cellcolor[HTML]{BEDACE}54.16\% & \cellcolor[HTML]{C7DFD5}46.44\% & \cellcolor[HTML]{F6FAF8}6.99\% & \cellcolor[HTML]{E5F0EC}21.18\% & \cellcolor[HTML]{FFFFFF}0.00\% \\
gpt-3.5-turbo-1106 & Random & \cellcolor[HTML]{A6CDBD}74.00\% & \cellcolor[HTML]{93C2AE}90.00\% & \cellcolor[HTML]{99C6B3}84.29\% & \cellcolor[HTML]{A2CBBA}77.14\% & \cellcolor[HTML]{ABD0C0}70.00\% & \cellcolor[HTML]{96C4B1}87.14\% & \cellcolor[HTML]{B0D2C4}65.71\% & \cellcolor[HTML]{ACD1C1}68.57\% & \cellcolor[HTML]{D2E5DD}37.50\% & \cellcolor[HTML]{E9F2EE}18.18\% & \cellcolor[HTML]{F7FBF9}5.88\% & \cellcolor[HTML]{F1F7F4}11.43\% & \cellcolor[HTML]{ACD1C2}68.47\% & \cellcolor[HTML]{97C5B2}86.28\% & \cellcolor[HTML]{B0D3C4}65.56\% & \cellcolor[HTML]{ADD1C2}68.07\% & \cellcolor[HTML]{D9E9E2}31.60\% & \cellcolor[HTML]{F6FAF8}6.99\% & \cellcolor[HTML]{F7FBF9}5.88\% & \cellcolor[HTML]{FBFDFC}2.71\% \\
\bottomrule
\end{tabular}
}
\end{table*}
